Semi-supervised reward learning for offline reinforcement learning

In offline reinforcement learning (RL) agents are trained using a logged dataset. It appears to be the most natural route to attack real-life applications because in domains such as healthcare and robotics interactions with the environment are either expensive or unethical. Training agents usually requires reward functions, but unfortunately, rewards are seldom available in practice and their engineering is challenging and laborious. To overcome this, we investigate reward learning under the constraint of minimizing human reward annotations. We consider two types of supervision: timestep annotations and demonstrations. We propose semi-supervised learning algorithms that learn from limited annotations and incorporate unlabelled data. In our experiments with a simulated robotic arm, we greatly improve upon behavioural cloning and closely approach the performance achieved with ground truth rewards. We further investigate the relationship between the quality of the reward model and the final policies. We notice, for example, that the reward models do not need to be perfect to result in useful policies.

==> old-text.tex <==
% \subsubsection{Reward models for different policy training}

% Finally, we would like to understand if using a specialized offline RL algorithm is better suited to be used in combination with learnt reward functions. 
% For this, we study the performance of D4PG algorithm instead of CRR on the same dataset, first, when having access to the ground truth. 
% The results for the four tasks are presented in the first row of \autoref{fig:CRR_vs_D4PG}. 
% Our findings match the results presented in the work of \cite{wang20CRR}: CRR is more efficient in offline learning. 
% Still, D4PG obtains reasonable scores in several task. 
% Next, we use CRR and D4PG with the learnt reward models from \textbf{MIL} and the results are presented in the second row of \autoref{fig:CRR_vs_D4PG} .
% While CRR with learnt reward still obtains high agent's scores, D4PG does not learn any good policy from this imprecise reward signal. 
% Our intuition to explain it is that CRR relies on reward values less than D4PG as it uses rewards only when learning critic, while D4PG needs reward signals both for actor and critic. 

% \begin{figure}
% \centering
%   \includegraphics[width=0.24\linewidth]{./images/5box0.pdf}
%   \includegraphics[width=0.24\linewidth]{./images/5insertion0.pdf}
%   \includegraphics[width=0.24\linewidth]{./images/5slide0.pdf}
%   \includegraphics[width=0.24\linewidth]{./images/5banana0.pdf}
%   \includegraphics[width=0.24\linewidth]{./images/5box1.pdf}
%   \includegraphics[width=0.24\linewidth]{./images/5insertion1.pdf}
%   \includegraphics[width=0.24\linewidth]{./images/5slide1.pdf}
%   \includegraphics[width=0.24\linewidth]{./images/5banana1.pdf}
%   \includegraphics[width=0.2\linewidth]{./images/5legend.pdf}
%   \caption{The effect of using learnt reward model with specialized offline RL algorithm. The returns of D4PG and CRR policies when using ground truth reward signal are shown in the first row, and the second row show their returns with \textbf{MIL} reward model. While CRR can learn a good policy from imprecise reward functions, D4PG fails completely.}
%   \label{fig:CRR_vs_D4PG}
% \end{figure}

%\subsubsection{Sparse of dense reward signal}

%When a reward function $R$ is trained, we can either use its output score directly for training an agent, or we can binarise it to be either $0$ or $1$ by thresholding the score at the $0.5$ value. 
%Our experiments\footnote{See the additional experiments.} have shown that despite the intuition that denser rewards (scores) should contain more information for training an agent than sparser rewards (binarised score), both methods perform equally well.
